Coends of higher arity

We specialise a recently introduced notion of generalised dinaturality for functors $T : (\mathcal{C}^\text{op})^p \times \mathcal{C}^q \to \mathcal{D}$ to the case where the domain (resp., codomain) is constant, obtaining notions of ends (resp., coends) of higher arity, dubbed herein $(p,q)$-ends (resp., $(p,q)$-coends). While higher arity co/ends are particular instances of "totally symmetrised" (ordinary) co/ends, they serve an important technical role in the study of a number of new categorical phenomena, which may be broadly classified as two new variants of category theory. The first of these, weighted category theory, consists of the study of weighted variants of the classical notions and construction found in ordinary category theory, besides that of a limit. This leads to a host of varied and rich notions, such as weighted Kan extensions, weighted adjunctions, and weighted ends. The second, diagonal category theory, proceeds in a different (albeit related) direction, in which one replaces universality with respect to natural transformations with universality with respect to dinatural transformations, mimicking the passage from limits to ends. In doing so, one again encounters a number of new interesting notions, among which one similarly finds diagonal Kan extensions, diagonal adjunctions, and diagonal ends.

==> preamble/diagram_environment.tex <==
%--- Diagram Environment
\makeatletter
\newcounter{diagramCounter}
\let\c@equation\c@theorem
\makeatother

\numberwithin{diagramCounter}{section}

\newenvironment{diagram}{%
	\setcounter{diagramCounter}{\arabic{equation}}
	\begin{equation}
		\refstepcounter{diagramCounter}%
		}{
	\end{equation}
}
\crefname{diagramCounter}{Diagram}{Diagrams}
%--- Diagram* Environment
\makeatletter
\newcounter{unnumberedDiagramCounter}
\AtBeginEnvironment{diagram*}{\stepcounter{unnumberedDiagramCounter}\let\c@equation\c@unnumberedDiagramCounter\def\theequation{\theunnumberedDiagramCounter}}
\makeatother

\numberwithin{unnumberedDiagramCounter}{subsection}

\newenvironment{diagram*}{%
	\setcounter{unnumberedDiagramCounter}{\arabic{equation}}
	\addtocounter{unnumberedDiagramCounter}{-2}
	\refstepcounter{unnumberedDiagramCounter}%
	\begin{equation*}
		}{
	\end{equation*}%
}
\crefname{unnumberedDiagramCounter}{Diagram}{Diagrams}



==> preamble/kusarigama.tex <==
\[
    \kgpq{q}{p}{G}\defeq
    \mathrlap{
        \begin{tikzpicture}[scale=0.8,baseline={(+0.0,+0.3)},anchor=base,opacity=0.25]
            % Sickle Gray
            \filldraw[gray!80] (0.2,0.99) -- (0.2,0.975) arc (81.1:49:1.35cm and 1cm) -- (0.5,0.825) -- (0.17,0.865);
            \filldraw[gray!50] (0.1685,0.855) -- (0.1685,0.855) arc (82.5:60:2cm and 1cm);
            \filldraw[gray!50] (0.18,0.89) -- (0.2,0.89) arc (82.5:60:1.5cm and 1cm);
            \filldraw[ultra thin, gray!50] (0.18,0.91) -- (0.45,0.857) -- (0.45,0.82) -- (0.1685,0.8425);
            % Handle Brown
            \filldraw[kusarigamaBrown] (0,0) -- (0.1,0.0) -- (0.2685,0.83) -- (0.1685,0.83) -- cycle;
            \filldraw[gray!90!black] (0,0) -- (0.1,0.0) -- (0.12,0.1) -- (0.02,0.1) -- cycle;
            % Chain
            \draw[thin,gray!90!black] (0.125,0.05) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black] (0.175,0.05) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black] (0.225,0.05) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black] (0.275,0.05) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black] (0.325,0.05) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black] (0.375,0.05) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={15:(0.425,0.0625)}] (0.425,0.0625) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={30:(0.475,0.085)}]  (0.475,0.085) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={40:(0.525,0.1175)}] (0.525,0.1175) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={40:(0.575,0.15)}]   (0.575,0.15) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={50:(0.615,0.19)}]   (0.615,0.19) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(0.6575,0.20)}]   (0.6575,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(0.725,0.20)}]    (0.725,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(0.775,0.20)}]    (0.775,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(0.825,0.20)}]    (0.825,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(0.875,0.20)}]    (0.875,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(0.925,0.20)}]    (0.925,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(0.975,0.20)}]    (0.975,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(1.025,0.20)}]    (1.025,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(1.075,0.20)}]    (1.075,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(1.125,0.20)}]    (1.125,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(1.175,0.20)}]    (1.175,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(1.125,0.20)}]    (1.125,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(1.175,0.20)}]    (1.175,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(1.125,0.20)}]    (1.125,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(1.225,0.20)}]    (1.225,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(1.275,0.20)}]    (1.275,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(1.325,0.20)}]    (1.325,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(1.375,0.20)}]    (1.375,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(1.425,0.20)}]    (1.425,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(1.475,0.20)}]    (1.475,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(1.525,0.20)}]    (1.525,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(1.575,0.20)}]    (1.575,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(1.625,0.20)}]    (1.625,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(1.675,0.20)}]    (1.675,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(1.725,0.20)}]    (1.725,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(1.775,0.20)}]    (1.775,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(1.825,0.20)}]    (1.825,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(1.875,0.20)}]    (1.875,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(1.925,0.20)}]    (1.925,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(1.975,0.20)}]    (1.975,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(2.025,0.20)}]    (2.025,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(2.075,0.20)}]    (2.075,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(2.125,0.20)}]    (2.125,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(2.175,0.20)}]    (2.175,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(2.125,0.20)}]    (2.125,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(2.175,0.20)}]    (2.175,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(2.125,0.20)}]    (2.125,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(2.225,0.20)}]    (2.225,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(2.275,0.20)}]    (2.275,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(2.325,0.20)}]    (2.325,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(2.375,0.20)}]    (2.375,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(2.425,0.20)}]    (2.425,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(2.475,0.20)}]    (2.475,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(2.525,0.20)}]    (2.525,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(2.575,0.20)}]    (2.575,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(2.625,0.20)}]    (2.625,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(2.675,0.20)}]    (2.675,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(2.725,0.20)}]    (2.725,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(2.775,0.20)}]    (2.775,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(2.825,0.20)}]    (2.825,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(2.875,0.20)}]    (2.875,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(2.925,0.20)}]    (2.925,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(2.975,0.20)}]    (2.975,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(3.025,0.20)}]    (3.025,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(3.075,0.20)}]    (3.075,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(3.125,0.20)}]    (3.125,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(3.175,0.20)}]    (3.175,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(3.125,0.20)}]    (3.125,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(3.175,0.20)}]    (3.175,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(3.125,0.20)}]    (3.125,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(3.225,0.20)}]    (3.225,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(3.275,0.20)}]    (3.275,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(3.325,0.20)}]    (3.325,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(3.375,0.20)}]    (3.375,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(3.425,0.20)}]    (3.425,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(3.475,0.20)}]    (3.475,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(3.525,0.20)}]    (3.525,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(3.575,0.20)}]    (3.575,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(3.625,0.20)}]    (3.625,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(3.675,0.20)}]    (3.675,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(3.725,0.20)}]    (3.725,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(3.775,0.20)}]    (3.775,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(3.825,0.20)}]    (3.825,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(3.875,0.20)}]    (3.875,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(3.925,0.20)}]    (3.925,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(3.975,0.20)}]    (3.975,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(4.025,0.20)}]    (4.025,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(4.075,0.20)}]    (4.075,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(4.125,0.20)}]    (4.125,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(4.175,0.20)}]    (4.175,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(4.125,0.20)}]    (4.125,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(4.175,0.20)}]    (4.175,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(4.125,0.20)}]    (4.125,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(4.225,0.20)}]    (4.225,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(4.275,0.20)}]    (4.275,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(4.325,0.20)}]    (4.325,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(4.375,0.20)}]    (4.375,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(4.425,0.20)}]    (4.425,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(4.475,0.20)}]    (4.475,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(4.525,0.20)}]    (4.525,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(4.575,0.20)}]    (4.575,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(4.625,0.20)}]    (4.625,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(4.675,0.20)}]    (4.675,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(4.725,0.20)}]    (4.725,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(4.775,0.20)}]    (4.775,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(4.825,0.20)}]    (4.825,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(4.875,0.20)}]    (4.875,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(4.925,0.20)}]    (4.925,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(4.975,0.20)}]    (4.975,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(5.025,0.20)}]    (5.025,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(5.075,0.20)}]    (5.075,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(5.125,0.20)}]    (5.125,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(5.175,0.20)}]    (5.175,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(5.125,0.20)}]    (5.125,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(5.175,0.20)}]    (5.175,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(5.125,0.20)}]    (5.125,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(5.225,0.20)}]    (5.225,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(5.275,0.20)}]    (5.275,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(5.325,0.20)}]    (5.325,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(5.375,0.20)}]    (5.375,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(5.425,0.20)}]    (5.425,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(5.475,0.20)}]    (5.475,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(5.525,0.20)}]    (5.525,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(5.575,0.20)}]    (5.575,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(5.625,0.20)}]    (5.625,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(5.675,0.20)}]    (5.675,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(5.725,0.20)}]    (5.725,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(5.775,0.20)}]    (5.775,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(5.825,0.20)}]    (5.825,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(5.875,0.20)}]    (5.875,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(5.925,0.20)}]    (5.925,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(5.975,0.20)}]    (5.975,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!70!black,rotate around={0:(6.025,0.20)}]    (6.025,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(6.075,0.20)}]    (6.075,0.20) ellipse (0.05cm and 0.02cm);
            \draw[thin,gray!90!black,rotate around={0:(6.125,0.20)}]    (6.125,0.20) ellipse (0.025cm and 0.01cm);
            %
            % Weight
            \begin{scope}
                \clip (6.345-0.25,0.15) -- (6.345-0.25,0.25) -- (6.405-0.25,0.25) -- (6.405-0.25,0.15) -- cycle;
                \draw[thin,gray!70!black,rotate around={90:(6.375-0.25,0.15)}]   (6.375-0.25,0.15) ellipse (0.05cm and 0.02cm);
            \end{scope}
            \filldraw[gray!70!black] (6.325-0.25,0.025) -- (6.345-0.25,0.15) -- (6.405-0.25,0.15) -- (6.425-0.25,0.025) -- cycle;
            \draw[black] (6.325-0.25,0.025) -- (6.345-0.25,0.15) -- (6.405-0.25,0.15) -- (6.425-0.25,0.025) -- cycle;
            % Handle
            \draw[black] (0,0) -- (0.2,0.99);
            \draw[black] (0,0) -- (0.1,0);
            \draw[black] (0.1,0) -- (0.2685,0.83);
            \draw[black] (0.02,0.1) -- (0.12,0.1);
            % Sickle
            \draw[thin,black] (-0.015,0) [partial ellipse=81.1:45:1.35cm and 1cm];
            \draw[thin,black] (-0.09,-0.15) [partial ellipse=82.5:59:2cm and 1cm];
            % Control Square
            %\draw[black] (0,0) -- (1,0) -- (1,1) -- (0,1) -- cycle;
        \end{tikzpicture}
    }%\mspace{-2mu}
    \int_{A\in\CatFont{C}}\ph_{A}\times\cdots\times\ph_{A}\times\ph^{A}\times\cdots\times\ph^{A}\pitchfork G^{A}_{A}.
\]


==> preamble/toc.tex <==
%▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓
%▓▓ ╔╦╗╔═╗╔╗ ╦  ╔═╗  ╔═╗╔═╗  ╔═╗╔═╗╔╗╔╔╦╗╔═╗╔╗╔╔╦╗╔═╗ ▓▓
%▓▓  ║ ╠═╣╠╩╗║  ║╣   ║ ║╠╣   ║  ║ ║║║║ ║ ║╣ ║║║ ║ ╚═╗ ▓▓
%▓▓  ╩ ╩ ╩╚═╝╩═╝╚═╝  ╚═╝╚    ╚═╝╚═╝╝╚╝ ╩ ╚═╝╝╚╝ ╩ ╚═╝ ▓▓
%▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓▓
\let\ToCFont\relax
\let\ToCBoldFont\relax
\newcommand{\ToCFont}{}
\newcommand{\ToCBoldFont}{\bfseries}

\newcommand{\TOC}{%
	{%
			\hypersetup{hidelinks}\tableofcontents
		}
}

\makeatletter
\newcommand \DotFill {\leavevmode \cleaders \hb@xt@ .33em{\hss .\hss }\hfill \kern \z@}
\makeatother

\definecolor{ToCGrey}{rgb}{0.0,0.0,0.0}% Gray doesn't look good with Computer Modern; let's change it to black
\definecolor{mainColor}{rgb}{0.82745098,0.18431373,0.18431373}
%\renewcommand{\cftsubsecfont}{\ToCFont\color{ToCGrey}}

%\renewcommand{\cftsecfont}{\ToCFont\color{black}\bfseries}
\usepackage{titletoc}


\titlecontents{part}
[0.0em]
{\addvspace{1pc}\color{mainColor}\large\bfseries\ToCBoldFont\text{Part }}
{\ToCBoldFont\bfseries\textcolor{mainColor}{\contentslabel{0.0em}}\hspace*{1.35em}}
{}
{\textcolor{mainColor}{{\hfill\ToCBoldFont\bfseries\contentspage\nobreak}}}
[]


\titlecontents{section}
[0.0em]
{\addvspace{1pc}}
{\ToCBoldFont\color{black}\bfseries\textcolor{mainColor}{\contentslabel{0.0em}}\hspace*{1.35em}}
{}
{\textcolor{black}{\textbf{\DotFill}{\ToCBoldFont\bfseries\contentspage\nobreak}}}
[]



\titlecontents{subsection}
[0.0em]
{}
{\hspace*{1.35em}\color{ToCGrey}\ToCFont{\contentslabel{0.0em}}\hspace*{2.1em}}
{}
{{\textcolor{ToCGrey}\DotFill}\textcolor{ToCGrey}{\ToCFont\contentspage}\nobreak}
[]

%\usepackage{sectsty}
%\sectionfont{\ToCFont}
%\subsectionfont{\ToCFont}
%\subsubsectionfont{\ToCFont}

%
%-------------
% We have to redefine these because of incompatibilities between titletoc and amsart
%-------------
\usepackage{titlesec}
\titleformat{\section}{\Large\bfseries}{\thesection. }{0em}{}
\titleformat{\subsection}{\large\bfseries}{\thesubsection. }{0em}{}
\titleformat{\subsubsection}{\bfseries}{\thesubsubsection. }{0em}{}
%\titleformat{\section}{\Huge\bfseries}{Kapitel \thesection.}{-110pt}{\newline}
%
% \usepackage{titletoc}
% \titlecontents{section}
% [3.8em] % ie, 1.5em (chapter) + 2.3em
%  {}
%  {\contentslabel{2.3em}}
%  {\hspace*{-2.3em}}
%  {\titlerule*[1pc]{.}\contentspage}


==> preamble/todonotes.tex <==
\usepackage[textwidth=2.5cm,colorinlistoftodos]{todonotes}
\usepackage{xcolor}
\definecolor{linkRed}{rgb}{0.780,0.007,0.000}
\definecolor{linkBlue}{rgb}{0.1,0.30,0.62}
\setlength{\marginparwidth}{2.5cm}
\setuptodonotes{fancyline, color=blue!30
}

\makeatletter
\newcommand\@todonotes@owner{default}
\define@key{todonotes}%
{owner}{\def\@todonotes@owner{#1}}

\newtoggle{ownerdefault}
\newtoggle{ownerB}

%--- Numbered Todo BEGIN
\newcounter{todocounter}
\newcommand{\ntodo}[2][]{\stepcounter{todocounter}\todo[#1]{\thetodocounter: #2}}
%--- Numbered Todo END

\newcommand{\todoFosco}[1]{
	{% 1st reviewer comment
			\ntodo[%
				inline,
				owner=default,
				author=\textcolor{white}{Fosco},
				%noline,
				caption={#1},
				color=linkBlue%
			]%
			{\color{white}{#1}}}
}

\newcommand{\prooftodo}[1]{
	% 2nd reviewer comment
	\ntodo[%
		inline,
		owner=B,
		%author=2nd Reviewer,
		noline,
		%caption={#1},
		color=linkRed%
	]%
	{\color{white}{#1}}
}


\renewcommand{\@todonotes@addElementToListOfTodos}{%
	\if@todonotes@colorinlistoftodos%
		\addtocontents{tdo}
		{%
			\protect\iftoggle{owner\@todonotes@owner}
			{%
				\protect\contentsline {todo}
				{\protect\fcolorbox{\@todonotes@currentbordercolor}%
					{\@todonotes@currentbackgroundcolor}%
					{\protect\textcolor{\@todonotes@currentbackgroundcolor}{o}}%
					\ \@todonotes@caption
				}{\thepage}{\@currentHref}%
			}{}%
		}%
	\else%
		\addcontentsline{tdo}{todo}{\@todonotes@caption}%
	\fi}%

\makeatother


==> preamble/widebar.tex <==
\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
\setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
\setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
\ifdim\ht0=\ht2 #3\else #2\fi
}
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
\begingroup
\def\mathaccent##1##2{%
%Enable nesting of accents:
\let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
\if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
\setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
\setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
\dimen@\wd\tw@
\advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
\divide\dimen@ 3
\@tempdima\wd\tw@
\advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
\divide\@tempdima 10
\advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
\ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
\rel@kern{0.6}\kern-\dimen@
\if#31
	\overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
	\advance\dimen@0.4\dimexpr\macc@kerna
	%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
	\let\final@kern#2%
	\ifdim\dimen@<\z@ \let\final@kern1\fi
	\if\final@kern1 \kern-\dimen@\fi
\else
	\overline{\rel@kern{-0.6}\kern\dimen@#1}%
\fi
}%
\macc@depth\@ne
\let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
\mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
\macc@set@skewchar\relax
\let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
\if#31
	\macc@nested@a\relax111{#1}%
\else
	%If the argument consists of more than one symbol, and if the first token is
	%a letter, use that letter for the computations:
	\def\gobble@till@marker##1\endmarker{}%
	\futurelet\first@char\gobble@till@marker#1\endmarker
	\ifcat\noexpand\first@char A\else
		\def\first@char{}%
	\fi
	\macc@nested@a\relax111{\first@char}%
\fi
\endgroup
}
\makeatother


==> sections/06-polyprof.tex <==
\section{Polyprofunctors}\label{sec:polyprofunctors}
\ansT{%
	What we need for polyprofunctors:
	\begin{enumerate}
		\item (\textcolor{FancyGreen}{$\checkmark$}) Fubini for associativity;
		\item (\textcolor{red}{$\times$})            Kusarigama lemma;
		\item (\textcolor{red}{$\times$})            A variant of the Kusarigama lemma justifying our composition law, like this one: let $\mathfrak{p}\colon\clC\polyproarrow{1}{2}\clD$ and $\mathfrak{q}\colon\clD\polyproarrow{3}{2}\CatFont{E}$ be polyprofunctors. Then
		      \[
			      \mathfrak{q}\procirc\mathfrak{p}
			      \defeq
			      \pqCoend{3}{3}{A\in\clD}\mathfrak{p}^{A,A}_{-}\times\mathfrak{q}^{-,-}_{A,A,A}\times\ph^{A}_{-}
			      \cong
			      \pqCoend{2}{3}{A\in\clD}\mathfrak{p}^{A,A}_{-}\times\mathfrak{q}^{-,-}_{A,A,A}.
		      \]
		      You'll notice that the $(3,3)$-coend above gives you a functor of variance $(2,2)$, while the $(2,3)$-coend gives you one of variance $(2,1)$. Figuring this out is part of the problem too.
	\end{enumerate}
}
\subsection{The bicategory of polyprofunctors}
\begin{definition}
	The bicategory $\cate{PolyProf}$ of \emph{polyprofunctors} is defined as follows:
	\begin{enumtag}{ppd}
		\item $0$-cells are pairs $(\clA,n), (\clB,m)$ where $\clA,\clB$ are small categories and $n,m\ge 0$ are integers.%
		%--- Begin Footnote ---%
		\footnote{%
			Note that with this definition $(\clA,p)\ne (\clA,q)$ for $p\ne q$.
		}%
		%---  End Footnote  ---%
		\item $1$-cells $\fkp : \clA \pto \clB$ are functors $\fkp : \clA^{-m}\times \clB^n \to \Set$ with the usual convention that $\clA^{-m}:= (\clA^\op)^m = (\clA^m)^\op$ is $m\ge 1$ (of course, $\clA^0=1$).
		\item $2$-cells $\alpha : \fkp \Rightarrow \fkq$ are usual natural transformations of functors.
	\end{enumtag}
	With these basic definitions,
	\begin{enumtag}{pps}
		\item the identity map of $(\clA,n)$ is just the hom functor $\hom_{\clA^n} : \clA^n \to \clA^n$;
		\item the composition of two polyprofunctors $\fkp : (\clA,p)\to (\clB,q)$ and $\fkq : (\clB,q) \to (\clC,r)$ is the polyprofunctor defined on objects as
		\[ \fkq \diamond \fkp : (\uA,\uC) \mapsto \pqCoend{q}{q}{B} \fkp^{\uA}_{\bsB}\times \fkq^{\bsB}_{\uC} \]
		and consequently from this on morphisms.
	\end{enumtag}
\end{definition}
In order to see that this is a well-posed definition, we shall show that the composition is associative up to canonical isomorphism, and that $\hom_{\clA^n}$ really works as an identity for $(\clA,n)$.

For associativity, consider three composable polyprofunctors $\clA \overset{\fkp}{\polyproarrow{p}{q}}\clB \overset{\fkq}{\polyproarrow{q}{r}} \clC \overset{\fkr}{\polyproarrow{r}{s}} \clD$
\begin{align*}
	(\fkr\diamond \fkq)\diamond \fkp & = \pqCoend{q}{q}{B} (\fkr\diamond \fkq)^{\bsB}_{\uD}\diamond \fkp_{\bsB}^{\uA}                                           \\
	                                 & \cong \pqCoend{q}{q}{B} \left(\pqCoend{r}{r}{C}\fkr^{\bsC}_{\uD}\times \fkq^{\bsB}_{\bsC}\right)\times \fkp_{\bsB}^{\uA} \\
	                                 & \cong \pqCoend{q}{q}{B} \pqCoend{r}{r}{C} \fkr^{\bsC}_{\uD}\times \fkq^{\bsB}_{\bsC}\times \fkp_{\bsB}^{\uA}             \\
	                                 & \cong \pqCoend{r}{r}{C} \pqCoend{q}{q}{B} \fkr^{\bsC}_{\uD}\times \fkq^{\bsB}_{\bsC}\times \fkp_{\bsB}^{\uA}
\end{align*}
and a similar expansion holds for $\fkr\diamond (\fkq\diamond \fkp)$.

For what concerns the identity, we shall show that for each $\fkp : \clA \polyproarrow{n}{m} \clB$,
\[ \fkp^{\uA}_{\uB} \cong \pqCoend{n}{n}{A} \fkp^{\bsA}_{\uB} \times \clA^n(\bsA,\uA) \]
and
\[ \fkp^{\uA}_{\uB} \cong \pqCoend{m}{m}{B} \fkp^{\uA}_{\bsB} \times \clB^m(\bsB,\uB) \]
Both identities hold by virtue of \cref{thm:kusarigama-lemma}.
\begin{example}[A case of study: polyprofunctors between sets]
	Let use consider the subcategory of $\cate{PolyProf}$ made by \emph{discrete} categories; this means we consider the category of sets and $|X|\times |Y|$-matrices $X \polyproarrow{m}{n} Y$ and ``generalised matrix product'' as composi; prendi tion.

	Such category can be canonically identified with the category whose objects are (finite powers of) finite sets $X^n,Y^m,\dots$ and whose morphisms $R : X,n \to Y,m$ are relations $R \subseteq X^n \times Y^m$.

	The composition rule is however different from the usual relation composition (that would amount to an iterated coend).
\end{example}
There's a looser notion of polyprofunctor, that fully exploits higher-arity coend calculus: \emph{semi-polyprofunctors} are triples $(\fkp,m,n) : \clA \pto \clB$, where we can compose $\fkp : \clA \polyproarrow{p}{q} \clB$ and $\fkq : \clB \polyproarrow{r}{s} \clC$ even when $r\ne q$, to obtain a profunctor $\clA^p \pto \clC^s$ by means of a $(q,r)$-coend.
\begin{definition}[A semicategory of polyprofunctors]
	We define $\cate{sPolyProf}$ as the structure having
	\begin{enumtag}{spp}
		\item 0-cells small categories $\clA,\clB,\clC$\dots
		\item 1-cells between $\clA$ and $\clB$ the triples $(\fkp,n,m)$, where $\fkp : \clA^n \pto \clB^m$ is a profunctor;
		\item 2-cells the natural transformations\dots
	\end{enumtag}
	\ans{\dots and here I got convinced that there is no such thing: what would a 2-cell of this kind be?
		$$\begin{tikzcd}[ampersand replacement=\&]
				\clA^n \ar[d]\ar[r, mid vert, "\fkp"]\& \clB^m\ar[d] \\
				\clA^r \ar[r, mid vert, "\fkq"']\& \clB^s
			\end{tikzcd}$$
		does not really make sense to me, because there is no point, from here, that prevents us to define a double category instead.
	}
\end{definition}


==> sections/temp-sandox.tex <==
\ansT{%
A \texttt{sandbox} where I'm trying to check that
\[
    \int^{A}\left(\ph^{X_{1}}_{A}\times\ph^{X_{2}}_{A}\times\ph^{A}_{Y}\right)\odot A
    \cong
    (\ph^{X_{1}}_{Y}\times\ph^{X_{2}}_{Y})\odot Y
\]%
indeed holds by computing $\ph\left(\int^{A}\left(\ph^{X_{1}}_{A}\times\ph^{X_{2}}_{A}\times\ph^{A}_{Y}\right)\odot A,-\right)$. Firstly, we have
\begin{align*}
    \ph\left(\int^{A}\left(\ph^{X_{1}}_{A}\times\ph^{X_{2}}_{A}\times\ph^{A}_{Y}\right)\odot A,-\right) &= \int_{A}\ph\left(\left(\ph^{X_{1}}_{A}\times\ph^{X_{2}}_{A}\times\ph^{A}_{Y}\right)\odot A,-\right)\\
                                                                                                        &= \int_{A}\left(\ph^{X_{1}}_{A}\times\ph^{X_{2}}_{A}\times\ph^{A}_{Y}\right)\pitchfork\ph\left(A,-\right)\\
                                                                                                        &= \int_{A}\left(\ph^{X_{1}}_{A}\times\ph^{X_{2}}_{A}\times\ph^{A}_{Y}\right)\pitchfork\ph^{A}_{-}\\
                                                                                                        &= \int_{A}\left[\ph^{X_{1}}_{A}\times\ph^{X_{2}}_{A}\times\ph^{A}_{Y},\ph^{A}_{-}\right].
\end{align*}
Now this end is an equaliser of the form
\[
    \Eq\left(
        \prod_{A\in\CatFont{C}}\left[\ph^{X_{1}}_{A}\times\ph^{X_{2}}_{A}\times\ph^{A}_{Y},\ph^{A}_{-}\right]
        \longrightrightarrows
        \prod_{f\colon A\to B}\left[\ph^{X_{1}}_{A}\times\ph^{X_{2}}_{A}\times\ph^{B}_{Y},\ph^{A}_{-}\right]
    \right),
\]%
where the first map is induced by precomposition with the map
\[
    \begin{tikzcd}[row sep={11.7em,between origins}, column sep={11.7em,between origins}, background color=backgroundColor, ampersand replacement=\&]
        \ph^{X_{1}}_{A}\times\ph^{X_{2}}_{A}\times\ph^{B}_{Y}
        \arrow[r,"\id\times\id\times\ph^{f}_{Y}"]
        \&
        \ph^{X_{1}}_{A}\times\ph^{X_{2}}_{A}\times\ph^{A}_{Y}\mrp{,}
    \end{tikzcd}
\]%
and the second map is induced by precomposition with
\[
    \begin{tikzcd}[row sep={11.7em,between origins}, column sep={11.7em,between origins}, background color=backgroundColor, ampersand replacement=\&]
        \ph^{X_{1}}_{A}\times\ph^{X_{2}}_{A}\times\ph^{B}_{Y}
        \arrow[r,"\ph^{X_{1}}_{f}\times\ph^{X_{2}}_{f}\times\id"]
        \&
        \ph^{X_{1}}_{B}\times\ph^{X_{2}}_{B}\times\ph^{B}_{Y}
    \end{tikzcd}
\]%
together with postcomposition with
\[
    \begin{tikzcd}[row sep={4.5em,between origins}, column sep={4.5em,between origins}, background color=backgroundColor, ampersand replacement=\&]
        \ph^{B}_{-}
        \arrow[r,"\ph^{f}_{-}"]
        \&
        \ph^{A}_{-}\mrp{.}
    \end{tikzcd}
\]%
What does it mean to equalise those maps?
\begin{enumerate}
    \item A map $\xi\colon E\longrightarrow\prod_{A\in\CatFont{C}}\left[\ph^{X_{1}}_{A}\times\ph^{X_{2}}_{A}\times\ph^{A}_{Y},\ph^{A}_{-}\right]$ is determined by the maps
        \[
            \left\{\xi^{A}\colon E\longrightarrow\left[\ph^{X_{1}}_{A}\times\ph^{X_{2}}_{A}\times\ph^{A}_{Y},\ph^{A}_{-}\right]\right\}_{A\in\Obj(\CatFont{C})}
        \]%
        These are assignments $e\mapsto\xi^{A}_{e}$, where
        \[
            \xi^{A}_{e}\left(\var[\phi]{X_{1}}A,\var[\psi]{X_{2}}A,\var[\theta]{A}Y\right)
            =
            \left[A\xlooongrightarrow{{\xi^{A}_{e}(\phi,\psi,\theta)}}-\right]\mrp{.}
        \]%
    \item That these are equalised means that
        \[
            \prod_{f}\xi^{B}_{e}(\phi,\psi,\theta\circ f)
            =
            \prod_{f}\xi^{A}_{e}(f\circ\phi,f\circ\psi,\theta)\circ f
        \]%
        holds, where those maps are
        \[
            \xi^{B}_{e}\left(\var[\phi]{X_{1}}B,\var[\psi]{X_{2}}B,\begin{bmatrix}A\\f\downarrow\\B\\\theta\downarrow\\Y\end{bmatrix}\right)
            =
            \var[]{A}{-}
        \]%
        and
        \[
            \xi^{A}_{e}\left(\begin{bmatrix}X_{1}\\\phi\downarrow\\A\\f\downarrow\\B\end{bmatrix},\begin{bmatrix}X_{2}\\\psi\downarrow\\A\\f\downarrow\\B\end{bmatrix},\var[\theta]{A}{Y}\right)\circ f
        \]%
\end{enumerate}
}
\tobecontinued
\ansT{}
